Approximation and Hardness for Token Swapping

Given a graph $G=(V,E)$ with $V=\{1,\ldots,n\}$, we place on every vertex a token $T_1,\ldots,T_n$. A swap is an exchange of tokens on adjacent vertices. We consider the algorithmic question of finding a shortest sequence of swaps such that token $T_i$ is on vertex $i$. We are able to achieve essentially matching upper and lower bounds, for exact algorithms and approximation algorithms. For exact algorithms, we rule out any $2^{o(n)}$ algorithm under the ETH. This is matched with a simple $2^{O(n\log n)}$ algorithm based on a breadth-first search in an auxiliary graph. We show one general $4$-approximation and show APX-hardness. Thus, there is a small constant $\delta>1$ such that every polynomial time approximation algorithm has approximation factor at least $\delta$. Our results also hold for a generalized version, where tokens and vertices are colored. In this generalized version each token must go to a vertex with the same color.

==> 4Approximation.tex <==
\section{$4$-Approximation}
Given a Token Swapping instance on graph $G$ we define the \emph{token permutation} as a permutation $\pi$ as follows. 
We say $\pi (i) = j$  if on vertex $i$ sits token $T_j$.

\begin{lemma}
  \label{lem:lower-bound}
Let $d(T_i)$ be the distance of token $T_i$ to the target vertex $i$.
Let $L$ be the sum of distances of all tokens to their target vertices:
 \begin{equation*}
   %\label{lower-bound}
L := \sum_{i=1,\ldots,n}{d(T_i)}.  
 \end{equation*}
Then any solution needs at least $L/2$ swaps.
\end{lemma}
\begin{proof}
 Every swap reduces $L$ by at most $2$.
\end{proof}
\begin{theorem}
	We can find in polynomial time a sequence of swaps that is  at most $4$ times worse than an optimal sequence of swaps, for the token swapping problem.
\end{theorem}
\begin{proof}



The permutation $\pi$ can be decomposed into a set of cycles. 
Let $L_C$ the sum of distances of tokens to their target vertices, for
all tokens of a cycle $C$.
The sum $L$ from
 Lemma~\ref{lem:lower-bound} 
 is the sum of $L_C$ over all cycles~$C$.
Thus it is sufficient to show how to resolve a cycle within at most $2L_C$ swaps without altering any other token.
\begin{observation}
	Given two tokens $T_i$ and $T_j$ with distance $d$ to another we can swap $T_i$ and $T_j$ without altering any other token with $2d-1$ swaps. 
\end{observation}
Just swap $T_i$ along the shortest path to $T_j$ and thereafter $T_{j}$ to the old position of $T_{i}$. On the way back all tokens on the path are put back into their old position.

	Let $C= i_1 i_2\ldots i_k $ be a cycle in $\pi$. We apply the observation on $T_{i_1}$ and swap it first with $T_{i_k}$ then with $T_{i_k-1}$ then with $T_{i_{k-2}}$ and so on. Finally we swap $T_{i_1}$ with $T_{i_2}$. Thereafter every token is at its target vertex and we used  \[(2d(T_{i_k}) -1)  +  (2d(T_{i_{k-1}}-1) + (2d(T_{i_{k-2}} -1) 
	+ \ldots + (2d(T_{i_{2}}-1) \, < \, 2L_C\] swaps. This finishes the proof.
\end{proof}


==> Application.tex <==
\section{Applications}

==> NPhardnessSpecialDisPath.tex <==
\section{NP-hardness of the Special Disjoint Path Problem}
\label{sec:disjoint-path}

For the NP-hardness proof of the Token Swapping problem, we will
study two auxiliary problems first. One of them is the 
\emph{Special Disjoint Path Problem}, we will define in the following.
 The input is a simple graph $G=(V,E)$ on
$n=t\cdot k$ vertices that are partitioned
into \emph{layers}
 $V_1,\ldots,V_t$ of uniform size $k$.
% , that is 
% $\lvert V_i \rvert = k \ \forall i = 1,\ldots,t$.
% Such a vertex class $V_i$ is also called layer.
 Edges can only go from $V_i$ to $V_{i+1}$.
In addition, we are given a bijection
 $\varphi \colon V_1 \longrightarrow V_t$, see Figure~\ref{fig:SDPPdef}. 
 \begin{figure}[htbp]%
 \centering
\includegraphics{SpecialDisPathDef}%
\caption{The input graph $G$ for the special
disjoint paths problem.}
%is partitioned into $V_1,\ldots,V_t$ 
%and edges are only between adjacent layers. We want to know if 
%there exists disjoint paths from $V_1$ to $V_t$, starting and ending
% at some predefined vertices.}%
\label{fig:SDPPdef}
\end{figure}

 The question is if there exists a set of disjoint paths 
 $P_1,\ldots,P_k$, such that 
 $P_i$ starts at $v_i \in V_1$ and ends at $\varphi(v_i)\in V_t$.
 
??? For the following sections the next Theorem and its proof are 
 vital as we will modify the reduction 
 described below. There might be simpler reductions, but we will 
 make use of the special structure of our reduction.
 
 \begin{figure}[htbp]%
 \centering
\includegraphics{BigPictureReduction}%
\caption{
Schematic drawing of
the disjoint graph instance $G_\psi$
for the \textsc{$3$-SAT} instance 
 $\psi = C_1\wedge \ldots \wedge C_4$, with 
$C_1 = \{x_1, \overline{x}_3,x_5\}$,
$C_2 = \{x_1, x_2, \overline{x}_6\}$, $C_3 = \{\overline{x}_2, x_3,\overline{x}_4\}$ 
and $C_4 = \{\overline{x}_1, \overline{x}_5,x_6\}$.
The paths go from top to bottom, and the layers are horizontal.
The horizontal rectangular boxes consist of three consecutive layers.
Each vertical line marked by $x_i$ stands for three paths, and
each vertical line marked by $C_j$ stands for a single path.
In each block of
 layers, the % variables and clause
 paths marked with a brown 
circle interact and all other paths just continue vertically.}
\label{fig:bigPicture}%
\end{figure}
 
 \begin{theorem}\label{thm:SDPPhard}
 	The Special Disjoint Path Problem is NP-complete.
 \end{theorem}
\begin{proof}
	
% 		\begin{figure}[hbt]
% 		\centering
% 		\includegraphics{SDPProblemReductionIdea}%
% 		\caption{Three variable gadgets are displayed. 
% 		The clause corresponds to $C = x_1 \wedge \overline{x_2} 
% 		\wedge x_3$. The red variable paths correspond to an 
% 		assignment $B$ setting all variables $x_1$, $x_2$ and $x_3$ 
% 		to false and thus only $\overline{x_2}$ satisfies $C$ and 
% 		thus the corresponding clause path displayed in blue 
% 		needs to go via $x_2$.  }%
% \label{fig:SDPPidea}%
% \end{figure}
  We reduce from \textsc{$3$-SAT}. Let $\psi$ be a formula in
  conjunctive normal form with $m$ clauses and $n$ variables.  We
  assume that no variable appears more than once in a clause.  The
  main idea of the reduction is to encode each variable and each
  clause by a path in an associated graph
  $G_\psi$ with $3m+4$ layers of size $m+3n$, see
  Figure~\ref{fig:bigPicture} for a schematic drawing.
For each clause $C$, three consecutive layers are reserved
  such that the interaction between the clause $C$ and its variables
  can take place in these layers and all other paths just continue to
  the next layer in an unambigious way. 

	
	Before we describe the details of the gadget that describes the interaction,
	we describe a simplified gadget, see Figure~\ref{fig:simplifiedInteraction}. 
	Assume clause $C$ interacts with variables $x_i$, $x_j$ and
        $x_k$. 
(Fig. UMBENENNEN!)
	  The path belonging to $C$ can only continue if it can go to one 
	  of the variables, and
the construction of the gadget ensures that $C$ can only go to a
variable if this variable makes the clause true.
 All other paths not belonging to the involved variables
	  just continue unambiguously.	
	\begin{figure}[htbp]
	  \centering
	  \includegraphics{simplifiedInteraction}
	  \caption{Clause $C$ interacts with variables $x_1$, $x_2$ and $x_3$. 
	  The path belonging to $C$ can only continue if it can go to one 
	  of the variables. All other paths not belonging to one of the variables
	  just continue unambiguously.}
	  \label{fig:simplifiedInteraction}
	\end{figure}

	The variable assignment is done with in the first two
	layers, see Figure~\ref{fig:SDPPconstruction}a. 
        For each variable $x_i$, we have three paths that we label by
        $x_i$, $d_i$, and $e_i$. In the first two layers
        $x_i$ and $d_i$ may swap places, and in the last two layers,
        they may swap back.

	The path of variable $x_i$ has two choices, which correspond
	to true and false. The other path is occupied by a 
	dummy-path, which might be later replaced, by yet another dummy-path.
% 	
	Let us describe the interaction between a variable and 
	its clause, see Figure~\ref{fig:SDPPconstruction}b--d. 
% 	
	Recall, the interaction between a clause and its variables
	is organized so that the clause path has to make a
	detour to one of its satisfying variables.
	We say clause $C$ picks variable $x$, if the clause 
	path goes through the gadget of variable $x$.
% 	
	Figure~\ref{fig:SDPPconstruction}~b) displays the the case that 
	$x_1$ satisfies $C$. The route that $x_1$ chose corresponds to a satisfying
	assignment. Accordingly, the clause path makes a detour via
	$x_1$ and a dummy-path ox $x_1$ occupies the free-vertex of $C$.
	Note that the dummy-path next to $x_1$ is switched,
	by a new one.
% 	
	Figure~\ref{fig:SDPPconstruction}~c) displays the  case that 
	$x_1$ does not satisfy $C$. Accordingly, the clause path 
	must go somewhere else. All dummy-paths stay with $x_1$.
	Note that the dummy-path next to $x_1$ gets replaced by a new one.
% 	
	Figure~\ref{fig:SDPPconstruction}~d) displays the  case that 
	$x_1$ does satisfy $C$, but $C$ nevertheless picks a different
	variable gadget to go to. Note also in this case the 
	dummy-path next to $x_1$ gets replaced by a new one.
% 	
	It is easy to check that no other combination can lead to
	a valid set of disjoint paths.
	
	
\begin{figure}[hbtp]
	\centering
	\includegraphics{3SATNEW2}%
	\caption{
The interaction between variable path for a variable $x_1$ and a
clause path $C$. We assume that $x_1$ occurs as a positive literal in~$C$.
The bijection between the first and the last layer is indicated by
corresponding labels.
%
a)~The variable $x_1$ (UMBENENNEN!) has the 
	choice between two paths. 
	The other path will be occupied by a 
	dummy-path $d$.
%
 This dummy-path might be replaced
	by another path, but another dummy-path.
	The variable path cannot switch between the
	left and right option before the very end.
	This choice between the left and right path corresponds
	to an assignment of the variable $x$.
	b)~Here the variable $x_1$ interacts with the clause 
	$C$. The route that $x_1$ chose corresponds to a satisfying
	assignment. Accordingly, the clause path makes a detour via
	$x_1$. 
	c)~$x_1$ does not satisfy $C$, but $C$ nevertheless picks a different
	variable gadget to go to. Note also in this case the 
	dummy-path next to $x_1$ gets replaced by a new one.
	d)~
	$x_1$ does satisfy $C$, but $C$ nevertheless picks a different
	variable gadget to go to. Note also in this case the 
	dummy-path next to $x_1$ gets replaced by a new one.}%
\label{fig:SDPPconstruction}%
\end{figure}
	
	Denote by $n(x)$ the number of clauses that the 
	variable $x$ appears in (Either in negated form or not.). 
	This is the number of total occurrences of $x$ as we assume
	that no variable appears in a clause twice. Then the number of
	dummy vertices for $x$ equals $n(x)+1$, as the dummy-path 
	next to the variable-path will be replaced for each 
	occurrence of $x$ in a clause. 
	Thus the number of vertices per layer $k$ equals $2n + 4m$:
	two vertices per variable and four vertices per clause.	
	The bijection $\varphi$ is implicitly given by the labels in 
	Figure~\ref{fig:SDPPconstruction}. 
	Note that this construction could be optimized, but our 
	purpose is to give a construction that can be described
	most easily and understandable.

	We denote by $I(\psi)$ the instance of the special 
	disjoint path problem generated in this way.
	It remains to show that $\psi$ is satisfiable if and only if 
	$I(\psi)$ is a yes-instance.
	
	[$\Rightarrow$] Assume there exists an assignment $A$
	 satisfying $\psi$. Then every variable-path and thus also
	 every dummy-path is prescribed as in 
	Figure~\ref{fig:SDPPconstruction}. In particular, every 
	clause-path finds a free vertex in at least one of 
	its corresponding variable-gadgets.
	
	[$\Leftarrow$] Assume now that we have given a set of disjoint
	paths from the top labels to the corresponding bottom labels.
	Then an assignment can be read off from the variable-paths 
	and every variable is set in a way that each clause is
	 satisfied by exactly one of its variables.
	\end{proof}

\newpage



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> NPhardnessSpecialDisPath2.tex <==
\section{NP-hardness of the Layered Disjoint Path Problem}
\label{sec:disjoint-path}

For the NP-hardness proof of the Token Swapping problem, we will study some simpler auxiliary problems first, as intermediate steps. One of them is the 
\emph{Layered Disjoint Path Problem}, defined as follows.
% 
\vspace{0.1cm}

 \noindent \textbf{Layered Disjoint Path Problem(LDPP)}
 \\ \noindent \textbf{input:} simple graph $G=(V,E)$ on
$n=t\cdot k$ vertices that are partitioned
into \emph{layers}
 $V_1,\ldots,V_t$ of uniform size $k$.
 Edges can only go from $V_i$ to $V_{i+1}$.
In addition, we are given a bijection
 $\varphi \colon V_1 \longrightarrow V_t$. 
 \\ \noindent \textbf{question:}
 does there exist a set of disjoint paths 
 $P_1,\ldots,P_k$, such that 
 $P_i$ starts at $v_i \in V_1$ and ends at $\varphi(v_i)\in V_t$?
 
 \vspace{0.1cm}
 

 
 \begin{lemma}\label{lem:LDPPhard}
 	There is a quadratic reduction from $3$SAT to the Layered Disjoint Path Problem.
 \end{lemma}
\begin{proof}
	
% 		\begin{figure}[hbt]
% 		\centering
% 		\includegraphics{SDPProblemReductionIdea}%
% 		\caption{Three variable gadgets are displayed. 
% 		The clause corresponds to $C = x_1 \wedge \overline{x_2} 
% 		\wedge x_3$. The red variable paths correspond to an 
% 		assignment $B$ setting all variables $x_1$, $x_2$ and $x_3$ 
% 		to false and thus only $\overline{x_2}$ satisfies $C$ and 
% 		thus the corresponding clause path displayed in blue 
% 		needs to go via $x_2$.  }%
% \label{fig:SDPPidea}%
% \end{figure}
  Let $\psi$ be a $3$CNF formula with $m$ clauses $C_1,\ldots,C_m$ and $n$ variables $x_1,\ldots,x_n$. We assume that no variable appears more than once in a clause. We will build a layered graph $G_{\psi}$ as in the definition of LDPP, such that each layer has $k = 4m+2n$ vertices and the total number of layers $t = 3m+4$.  The main idea of the reduction is that $n$ of the $k$ disjoint paths represent a variable assignment of all the variables and $m$ paths represent clause satisfiability. The remaining \emph{filler paths} serve to cover the remaining vertices. For each clause $C$, three consecutive layers are reserved such that the interaction between the clause $C$ and its variables can take place in these layers and all other paths just continue to the next layer in an unambiguous way. For each variable $x$, we have a path, denoted by \emph{$x$-path}, symbolizing its assignment.  Similarly, for each Clause $C$, we have a path, denoted by \emph{$C$-path}, symbolizing its satisfiability.   
  Further denote by $n(x)$ the number of occurrences of $x$ in the formula $\psi$. Then for each variable, we introduce $n(x)+1$ filler paths. The filler paths are needed for two purposes. The first is the assignment of the variables. The assignment of a variable $x$ is represented by the vertex in the second layer that the $x$-path choses. The filler path must pick the vertex that was not chosen by the $x$-path. We say this filler-path is \emph{active}. 
  The second purpose of filler paths is to help for the variable clause interaction. In this interaction the active filler path will become inactive and is replaced by another inactive filler path. At all times there is exactly one filler path for each variable active and a filler path that was active once will never be active again.
  Before, we will explain the gadgets for the variable  assignment and the variable clause interaction, see Figure~\ref{fig:bigPicture} for a schematic simplified drawing of the graph $G_{\psi}$, for some specific $\psi$.
  \begin{figure}[htbp]%
  \centering
  \includegraphics{BigPictureReduction2}%
  \caption{
    Schematic drawing of the disjoint graph instance $G_\psi$ for the \textsc{$3$-SAT} instance  $\psi = C_1\wedge C_2$, with $C_1 = \{x_1, \overline{x}_2,x_4\}$ and $C_2 = \{\overline{x}_1, x_3, \overline{x}_5\}$. The paths go from top to bottom, and the layers are horizontal. The horizontal rectangular boxes consist of three consecutive layers. Each vertical line marked by $x_i$ symbolizes the start of the $x_i$-path, and each vertical line marked by $C_j$ symbolizes the start of the $C_j$-path. In each block of layers, the paths marked with an orange circle interact and all other paths just continue vertically. The active filler path is marked green.}
  \label{fig:bigPicture}%
\end{figure}
  
  Let us now describe the representation of the variable assignment of variable $x$. It consists of two parallel paths in the graph $G_{\psi}$. One symbolizes the assignment true and the other the assignment false. The idea is that the $x$-path chooses in the beginning which path to take. The other path will be taken by the active filler path, see Figure~\ref{fig:variableAssignment}.
  \begin{figure}[htbp]%
  \centering
  \includegraphics{variableAssignment}
	\caption{The variable assignment gadget.}%
  \label{fig:variableAssignment}%
\end{figure}
  We think of the $x$-path as going from layer to layer. In this process, the filler path that is active will change at every variable clause interaction gadget, which involves the corresponding $x$-path.

  Now, let us turn our attention to the variable clause interaction gadget. To simplify matters let us remark first that the gadget does not care so much whether a variable $x$ appears in normal or negated form in a clause $C$. One of the assignment paths that is visited by $x$ corresponds to a satisfying assignment for $C$ and the other does not satisfy $C$. We denote the first path as positive path and the second as negative path.
  
  Further, we note that a clause interacts with three variables, but the interaction to each variable is exactly the same. Thus we describe only one such interaction. See Figure~\ref{fig:VarClauseInteractionProof}~a) for a drawing of the variable clause interaction gadget reduced to one variable. The left part of the gadget is present for every involved variable and the right part of the gadget is shared by all variables of that specific clause.
  
  See Figure~\ref{fig:ExplicitExample2} for a drawing of the graph $G_{\psi}$, for the same $\psi$ as in Figure~\ref{fig:bigPicture}. The general rule for the definition of the bijection $\varphi$ from the first to the last layer can be read of easily from Figure~\ref{fig:ExplicitExample2}.
    \begin{figure}[htbp]%
  \centering
  \includegraphics{Case1VarClauseInteract}%
	\caption{a) The variable clause interaction gadget 
	b) Case 1 of Claim~\ref{clm:varClause}
	c) Case 2 of Claim~\ref{clm:varClause}
	d) Case 3 of Claim~\ref{clm:varClause}
	}%
  \label{fig:VarClauseInteractionProof}%
\end{figure}
  To understand the variable clause interaction gadget we summarize its potential behaviour in Claim~\ref{clm:varClause}
  \begin{claim}\label{clm:varClause}
      Given a variable clause interaction gadget with one actice filler path, one inactice filler path, one $x$-path and one $C$-path there are exactly three ways these paths pass through the gadget.
      \begin{enumerate}
       \item the $x$-path uses the positive path and the $C$-path visits vertex $v$.
       \item the $x$-path uses the positive path, but the $C$-path does not visits vertex $v$.
       \item the $x$-path uses the negative path and the $C$-path does not visits vertex $v$.
      \end{enumerate}
	In all three cases the active and inactive filler paths change role and the $x$-path does not change its assignment.
  \end{claim}
  \begin{proof}%[proof of Claim~\ref{clm:varClause}]
    From Figure~\ref{fig:VarClauseInteractionProof}~b),~c) and d) it is easy to see that all the described options are indeed possible. The $x$-path is displayed blue, the filler paths are displayed in yellow and the $C$-path is displayed red.
    It is easy to check that no other behavior will lead to a valid transversals  of the gadget by disjoint paths. The $x$-path must stay on one of the assignment paths, because of the global construction and as there is no way to switch from one assignment path to the other, it will just stay on the assignment path it started from. The inactive filler path must go to either assignment path and become active, as the only options. Thus the active filler path must leave the assignment path and become inactive.
    In the cases displayed in Figure~\ref{fig:VarClauseInteractionProof}~c) and~d) the $C$-path will go to some other variable and the filler path of that variable will go to vertex $w$. 
  \end{proof}
  
  Now, we are ready to finish the proof. Assume that we have given a $3$CNF formula $\psi$ with $n$ variables and $m$ clauses. Further let $G_\psi$ be the layered graph as described above and $\varphi$ be the corresponding bijection of the first and last layer.
  
  Assuming that $\psi$ is satisfiable we show first that there exist $4m+2n$ disjoint paths from the first to the last layer. Let $A$ be a satisfying assignment of $\psi$. Then for each variable $x_i$ the $x_i$-path chooses to go to the corresponding assignment path. Further for each clause $C$ there will be one $x$-path that uses the assignment path that is positive for that clause. Thus each $C$-path has a variable that it can enter as in Figure~\ref{fig:VarClauseInteractionProof}~b). Because the filler paths always swap each path will end at the vertex indicated by $\varphi$.
  
  Reversely, we consider the case that there exist a set of $4m+2n$ disjoint paths with correct start and end vertices. These paths naturally define an assignment of the variables. Then for each $C$-path there exists an $x$-path such that this $C$-path can enter the corresponding gadget. Which is only possible if the variable assignment of $x$ satisfies the clause $C$, as the $x$-path cannot change its assignment. Thus there exists an assignment that satisfies $\psi$.
\end{proof}  
\begin{figure}[hbtp]
	\centering
	\includegraphics[]{ExplicitExample2}%
	\caption{A drawing of $G_{\psi}$}
\label{fig:ExplicitExample2}%
\end{figure}

\begin{figure}[hbtp]
	\centering
	\includegraphics[]{ExplicitExample2Assigned}%
	\caption{A drawing of $G_{\psi}$ together with a valid set of paths in white.}
\label{fig:ExplicitExample2Assigned}%
\end{figure}
The above proof uses at many points unnecessary vertices. These are used in order to enforce the layer structure and keep the graph $G_{\psi}$ as simple as possible. We want to use the reduction also to conclude lower bounds on the running time with the help of the exponential time hypothesis. Therefore, we have to relax the condition of the layer structure in order to make the above reduction linear.

\vspace{0.1cm}

 \noindent \textbf{Special Disjoint Path Problem(SDPP)}
 \\ \noindent \textbf{input:} 
 A directed graph $G=(V,E)$ on $n$ vertices that are partitioned into \emph{layers} $V_1,\ldots,V_t$ such that:
 \begin{enumerate}
  \item Layer $V_1$ and $V_t$ have exactly $t$ vertices and every other layer has at most $t$ vertices. 
  \item For every edge $vw$ with $v\in V_i$ and $w\in V_j$ holds $i<j$.
  \item Every vertex $v\in V_i$ has either indegree $1$ or all ingoing edges are incident to vertices in layer $V_{i-1}$.
 \end{enumerate}
 In addition, we are given a bijection $\varphi \colon V_1 \longrightarrow V_t$. 
 \\ \noindent \textbf{question:}
 Can $G$ be partitioned into disjoint paths $P_1,\ldots,P_k$, such that $P_i$ starts at $v_i \in V_1$ and ends at $\varphi(v_i)\in V_t$?
 
 \vspace{0.1cm}
 
  \begin{corollary}\label{cor:SDPPhard}
    There exists a \emph{linear} reduction from $3$SAT to the Special Disjoint Path Problem.
  \end{corollary}
  \begin{proof}
    Let $G_\psi$ be the graph as in Lemma~\ref{lem:LDPPhard}. We construct a graph $G_\psi'$ as in the definition of SDPP. The bijection $\varphi$ is not changed. Consider the set $S\subseteq V$ of vertices $v$ with $deg(v)=2$. The set $S$ forms a collection of disjoint paths. Remove all interior vertices of each path and connect the endpoints of the paths by an edge. Further direct all edges in the obvious way. We will show that the number of remaining vertices is linear. All vertices $v$ that remain have either $deg(v)>2$, are adjacent to a vertex $w$ with $deg(w)>2$ or are in the first or last layer. The number of vertices in the theses layers is linear. All other vertices are part of some gadget. Each gadget has constant size and we use a linear number of gadgets. Thus the total number of vertices is linear.
    
    It is easy to see that $G_\psi'$ satisfies the conditions in SDPP.
    Further, let $P_1,\ldots, P_k$ be a set of disjoint paths of $G_\psi$.
    Then these paths define paths $P_1',\ldots, P_k'$ covering all vertices of $G_\psi'$, by contracting appropriate edges.
    The reverse direction holds as well. To see this note that, whenever $P_i'$ uses an edge $uv$ from two non-adjacent layers in $G_\psi'$ then there exists a unique path from $u$ to $v$ in $G_\psi$.
  \end{proof}

    
  



\newpage



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> NPhardnessUnRelaxed.tex <==
\section{Even Permutation Networks}\label{sec:permutation}

TILL: Under Construction


Consider a family of token swapping instance $I(\pi)$, which depends on a permutation $\pi$ from some specific set of input vertices $V_\textup{in}$ to some set of output vertices $V_\textup{out}$. The permutation $\pi$ specifies, for each token initially on $V_\textup{in}$ the target vertex in $V_\textup{out}$. For every other token, the target vertex is independent of $\pi$. If the optimal number of swaps to solve the $I(\pi)$ is the same for every \emph{even} permutation $\pi$, we call this family an \emph{even permutation network}, see Figure~\ref{even-perm}. (We will later further require that it takes more swaps for odd permutations.) 
Recall that a permutation is even, if the number of inversions of the permutation is even.


(Note that realizing \emph{all} permutations at the same cost is impossible, since every swap changes the parity, and hence all permutations reachable by a given number of swaps have the same parity.)  Rather than verifying that all candidate permutations that
  are used in our reduction (Figure~\ref{fig:clause}b--d) have the
  same parity (which is actually the case) we use the simple trick of
  doubling the whole input graph before attaching the permutation
  networks. We thereby ensure that realizing even permutations is sufficient:
  the product of two permutations of the same parity is always even.


  

\begin{figure}
  \centering
  \includegraphics{even-perm}
  \caption{The interface of a permutation network PN}
  \label{even-perm}
\end{figure}

% \begin{figure}
%   \centering
%   \includegraphics{attach}
%   \caption{Attaching a permutation network to let the filler tokens
%     destined for $V_{j}$ arrive at their final destinations $V_j'$.
% The small ``vertical'' network in this figure represents the network constructed in
% Lemma~\ref{thm:coloredhard}.}
%   \label{attach}
% \end{figure}


The constructed network has $n$ input vertices $V$ and $n$ output
vertices $V'$, plus $O(n^3)$ inner vertices $V_{\mathrm{PN}}$.  For
each token on $ V_{\mathrm{PN}} \cup V'$, a fixed target vertex in
$V \cup V_{\mathrm{PN}}$ is defined. The target vertices of~$V$
lie in $V'$ but
are still unspecified.
The tokens
on $V$ are filler tokens for the graph to which PN is attached,
but for the purposes of constructing PN, we will classify them as \emph{input
tokens},
and the filler tokens are all remaining tokens.

\begin{lemma}\label{lem:PermutationNetworks}
  For every $n$, there is a permutation network
$\mathrm{PN}%=\mathrm{PN}_n
$ with $n$ input vertices $V$, $n$ output
vertices $V'$,
and $O(n^3)$ additional vertices
$V_{\mathrm{PN}}$, which has the following properties, for some value $T$\textup:
\begin{itemize}
\item For every target assignment $\phi$ between the inputs
 $V$ and the outputs
 $V'$ that is an even permutation, there is a swapping sequence of
 length $T$.
%\item For every target assignment $\phi$
% that is an odd permutation, every swapping sequence has length at
% least  $T+1$.
\item For any other target assignment, the shortest realizing sequence
  has length at least $T+1$. This includes any extension $G'$ 
%of the network PN
 which is the union of PN with another graph $H$ that
  shares only the vertices $V$ with PN, and in which the starting
  positions of the tokens assigned to $V'$ may be anywhere in 
$H$.
%$G'$ \textup(excluding
%  $V_{\mathrm{PN}}\cup V'$, since the targets of these vertices are
%  already specified in PN\textup).
\end{itemize}
\end{lemma}
The second clause concerns all
assignments between
 $V$ and
 $V'$ that are odd permutations, but also all other conceivable
 situations where the tokens destined for $V_i$ do not end up in $V_i$
 but somewhere else in the ``vertical'' network $H$ of
Figure~\ref{attach}. The lemma confirms that such non-optimal
solutions for $H$ cannot be combined with solutions for PN to yield
better swapping sequences than the ones for which the network was designed.

\begin{proof}
The network will be built up hierarchically from small gadgets.
Each gadget is built in a layered manner, similar to the graphs
in
Section~\ref{sec:disjoint}, but subject to the following
slightly different rules, see Figure~\ref{fig:transpose}
for an example.
\begin{enumerate}
\item There is a strict layer structure: The vertices are partitioned
  into layers $V_1,\ldots,V_t$ of the same size.
\item Each gadget has its own input layer $V=V_1$ at the top and its
  output layer $V'=V_t$ at the bottom,
just as the overall network PN.
\item
\label{assign-unique}
 Edges may run
 between two vertices of
  the same layer
(\emph{horizontal  edges}), or between adjacent layers
(\emph{downward edges}).
\item Every vertex has at most %exactly
 one neighbor in the successor layer 
and at most one neighbor in the predecessor layer.
%, with the obvious exceptions for the
%vertices in the boundary layers $V$ and $V'$.
\end{enumerate}
The goal is to bring the input tokens from the input layer $V$ to the output
layer~$V'$. By Rule \ref{assign-unique}, the cheapest conceivable way to
achieve this % to bring the tokens from $V$ to $V'$
is by using only the downward edges,
and then every such edge is used precisely once.

The gadget in Figure~\ref{fig:transpose} has an additional input
vertex $a$ with a fixed destination, indicated by the label~$a$.
This assignment forces us to use also horizontal edges, incurring some
extra cost as compared to letting the input tokens travel only
downward.

We will be able to check in every case that
we only need to consider candidate 
swapping sequences in which
every downward edge is used precisely once. (CHECK THIS!!)
This has the following consequences.
\begin{enumerate}
\item 
We can compare the cost of swapping sequences by counting the
horizontal edges used.
\item Each of the filler tokens,
which fill the vertices of the graph,
 % except the ones from $V$ that trickle down, 
  moves one layer up to a fixed target location. Thus, the problem
  that haunted us initially, namely that we cannot predict the final
  position of all the auxiliary filler tokens that fill the network,
  does not reappear at this level.
\end{enumerate}
%
Let us now look at the example of Figure~\ref{fig:transpose}.
It has three inputs 1,2,3 that connect the gadget with other gadgets, plus
an additional input $a$ with a specified target.
The initial vertex of $a$ and the target vertex of $a$ are not
connected to other parts of the graph.
The possible permutations of 1,2,3 that arise on the output are in the table
below the network, together with the number $\#h$ of used horizontal edges
(i.e., the relative cost).

Let us check this table.
To get the token $a$ into the correct target position, we must get it from the
fourth track to the third track, using (at least)
two horizontal edges ($A,B$ or $D,E$ or $A,E$). With this minimum
cost of 2, we reach the identity permutation $1,2,3$. If we use edge
$C$, we can also reach the permutations $3,2,1$ (together with $A,B$)
and $2,1,3$ (together with $D,E$), at a cost of 3. All other possibilities
that bring the tokens from $V$ to $V'$ and bring $a$ to the correct
target cost more, including ``crazy'' swapping sequences where the
tokens $1,2,3,a$ make intermediate upward moves.

In summary, the gadget can either realize the identity permutation, or
it can swap 1 with one of the other tokens at an extra cost of~1. 
We
call this the swapping gadget, and we will  symbolize it likw % as shown
in the right part of Figure~\ref{fig:transpose}, omitting the
auxiliary token~$a$.

\begin{figure}
  \centering
  \includegraphics{transpose}
  \caption{The gadget for swapping 1 with 2 or 3.  The number of
    horizontal edges used is denoted by $\#h$.}
  \label{fig:transpose}
\end{figure}


The next gadget is the shift gadget, which is composed of two
swapping gadgets as shown in Figure~\ref{fig:shift}.
When putting together gadgets, the tracks must be filled up with
vertices on straight segments to maintain the strict layer structure, but we
don't show these
 trivial paths in the pictures.

We have a token $b$ with a fixed target, which is not connected to the
rest of the graph. To bring $b$ from the first track to the fourth
track and hence to the target, we cannot use the identity permutation
in % either of
 the % two
 swap gadgets;
in both swapping gadgets, we must use one of the more expensive
swapping choices.
There are two choices that put $b$ on the correct target:
The choice ``swap $b\leftrightarrow2 $ and then swap $b\leftrightarrow 3$'' leads to the identity
permutation $1,2,3$.
The choice ``swap $b\leftrightarrow1$ and then swap
$b\leftrightarrow3$'' leads to the cyclic shift $3,1,2$.
We thus conclude that this gadget has two minimum-cost solutions:
The identity, or a cyclic shift to the right.
%
The shift gadget is symbolically drawn as a rectangular box as shown
in the right part of Figure~\ref{fig:shift},
indicating the optional cyclic shift.


\begin{figure}
  \centering
  \includegraphics{shift}
  \caption{The gadget for an optional cyclic shift of 1,2,3 by one position}
  \label{fig:shift}
\end{figure}

From the shift gadget, we can now build the whole permutation network
PM. The idea is similar to the realization of a permutation as a product of
adjacent transpositions, or to the bubble-sort sorting network.
%
Figure~\ref{fig:end} shows how a cascade of $n-1$ shift gadgets can
bring any input token to the last position.  We add a cascade of $n-2$
shift gadgets that can bring any of the remaining tokens to the
$(n-1)$-st position, and so on. In this way, we can bring any desired token
into the $n$-th, $(n-1)$-st, \dots, 3rd position. The first two
positions are then fixed, and thus we can realize half %$1/2$
of all permutations,
namely the even ones.
% We have argued above that all realizable
%permutations have the same parity, and we see that the identitiy
%permutation is realizable. We conclude that we can realize every even
%permutation.
\end{proof}

\begin{figure}
  \centering
  \includegraphics{to-end}
  \caption{The gadget for bringing any desired token to the last position}
  \label{fig:end}
\end{figure}






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> notation.tex <==
\section{notation}

\begin{enumerate}
\item target vertex of a token:
the vertex a token wants to go to.
\item  $d(t)$ the distance of a token to its target vertex.
\item  We say a swap sequence $(s_1,\ldots,s_l)$ is a \emph{happy cycle} swap if the edges involved in the swaps form a cycle of length $l+1$ and every token reduces its distance  to their respective target vertex by exactly $1$.
\item A swap is called \emph{unhappy} if one of the tokens already is on its target vertex and the other token reduces its distance to its target vertex.
\item optimal sequence of swaps: sequence of swaps with minimum length from the start placement to the target placement.
\item $L$: $L$ the sum of distance of the tokens to its target vertices
(Maybe we can use this letter for this variable.)
\item $Opt$:  $Opt$ denotes the minimum number of swaps
(Maybe we can use these letters for this variable.)
\item Definition of the special disjoint path problem:
We define first what we mean with a \emph{layer graph}.
A graph $G = (V,E)$ is a layer graph if  $V = V_1\cup\ldots\cup V_t$ and $|V_i| = k$ for all $i$. These sets are called \emph{layers}. Further every edge is incident to two adjacent layers $V_i$ and $V_{i+1}$ and $i = 1,\ldots, t-1$. 
The \emph{special disjoint path problem} has as input a layer graph and a perfect matching $M$ not part of $G$ between the vertices of layer $V_1$ and layer $V_t$.
We ask if there exists $k$ disjoint path from $V_1$ to $V_t$ that connects each vertex with its matched partner.
(TM: This definition belongs to the introduction maybe.)
\item \emph{relaxed token swapping problem}: More precisely, each token $T_i$ has a \emph{color} $C_i$,
each vertex $j$ has a color $D_j$, and the goal is to
let each token arrive at a vertex of its own color.
We call this the \emph{relaxed token swapping problem}. 
\item Given a Token Swapping instance on graph $G$ we define the \emph{token permutation} as a permutation $\pi$ as follows. 
We say $\pi (i) = j$  if on vertex $i$ sits token $T_j$.
\end{enumerate}

==> nphardnessunrelaxed-old.tex <==
\section{NP-hardness}
We are now ready to prove the main result.

\begin{figure}[htbp]
	\centering
\includegraphics{TokenReductionGadget}%
\caption{The gadget belonging to the clause $C = \{x , \overline{y}\}$.}%
\label{fig:TRG}%
\end{figure}

\begin{theorem}\label{thm:main}
	The token swapping problem is NP-complete.
\end{theorem}
\begin{proof}

	The general structure of the proof is simple. We reduce from
	$1$in$3$-SAT to the token swapping problem in three
	steps. Let $\varphi$ be an instance of $1$in$3$-SAT.
	
	Step $1$ is the reduction from $1$in$3$-SAT to the 
	special disjoint path problem as described in 
	Theorem~\ref{thm:SDPPhard}.
	We denote such an instance of the special disjoin path
	problem by $SDP(\varphi)$

	Step $2$ is the reduction from the special disjoint path
	problem to the colored token swapping problem as described
	in Theorem~\ref{thm:coloredhard}.
	We denote an instance of the colored token swapping
	problem, which is constructed in this way, by $CTS(\varphi)$.
	
	Step $3$ takes an instance $CTS(\varphi)$ of the colored
	token swapping problem and gives every token a distinct color
	and specifies the target vertex of the ordinary tokens.
	Recall that the ordinary tokens did not have a unique color.
	Additionally, some subtle modifications of the underlying graph
	will be added, as it would be
	otherwise difficult for the ordinary tokens to reach its target 
	vertex. 
	Also the threshold $T$ must be increased, so that those
	additional swaps taking care of the ordinary tokens
	are possible.
	We denote an instance of the colored token swapping
	problem, which is constructed in this way, by $TS(\varphi)$.
	
	To show the correctness of this construction is tedious, because
	it might be possible to cheat. Here, cheating means that
	we cannot find a satisfying assignment of $\varphi$ 
	corresponding to a sequence of swaps solving $TS(\varphi)$.
	Some of our modifications are only made to make cheating 
	sufficiently expensive.
	Recall that in Theorem~\ref{thm:coloredhard} 
	cheating was impossible, because every real token made 
	exactly $t-1$ swaps and if the real tokens swapped along
	disjoint paths all ordinary tokens are at its right 
	position.
	Now it is possible that one real token makes a few more 
	swaps, if this can be compensated by some ordinary tokens 
	making fewer swaps. Thus this is to be prevented.
 	
 	
 	
	The remainder of the proof, will describe how to do
	the modifications and thereafter prove by exhaustive case
	distinction that cheating is not worth the effort.
	
	
	
	To start our discussion, consider a clause $C$ 
	with one of its variables,
	say $x$, as in Figure~\ref{fig:SDPPconstruction}.
	Studying the interplay of $x$ and $C$, we notice
	that only two possibilities arise. Either $x$ satisfies
	$C$ or it does not. In particular, if there are two variables
	$x$ and $y$ than the tokens belonging to the $x$ gadget and
	the tokens belonging to the $y$ gadget do not swap 
	with each other.
	Thus it is sufficient to restrict out attention to
	a clause $C$ with two variables and for easier drawing we
	choose $C = \{x, \overline{y}\}$. 
	A drawing can be seen in Figure~\ref{fig:TRG}.
	Ignore at first the dotted lines. The graph displayed
	in Figure~\ref{fig:TRG} is nothing else than the
	construction of Theorem~\ref{thm:SDPPhard} applied to the 
	clause $\{x, \overline{y}\}$ drawn conveniently.
	Note that the gadget for $x$ and $\overline{y}$ is symmetric.
	So we do not care so much whether $x$ is set to 
	true or to false, but only if $x$ satisfies $C$ 
	or not.
	
	We further specify that every token on the top
	row has as target vertex the vertex on the bottom row
	with the same label. Every other token has the vertex just
	above it as target vertex. (It is easy to adopt these rules
	for a clause with three literals, but we don't draw it 
	as the clutter would make it unreadable.)

	
	We will modify this construction later even more.
	To see the purpose of the dotted edges consider the
	satisfying assignment of the variables $x = F$ and $y = F$
	and the corresponding honest paths displayed in
	Figure~\ref{fig:desPath}.

	We call a swap not involving a real token moving from 
 	one layer to the next layer an \emph{extra swap}. As we know every
 	real token must make at least $t-1$ swaps from the first 
 	to the last layer, we are only interested in extra swaps.
	
	Consider the green path of token labeled $x$. As the 
	start vertex and the target vertex are in different columns 
	$x$ has to switch its column exactly once. This is possible 
	when moving from the first to the second layer
	and it is possible  when moving from the penultimate to the last 
	layer. Which of the cases apply depends on whether the variable
	$x$ is assigned to true or false. 
	When the token $x$ switches the column one ordinary token
	has to do an extra swap, which we call \emph{extra outside swap}.
	In total, we have $n$ extra outside swaps. (Recall $n$ denotes 
	the number of variables in $\varphi$.) The name outside stems from
	the fact that this extra swap will happen at the very top
	or at the very bottom, that is outside of any clause-gadget.
	Otherwise, when we talk about an extra swap it will be always
	an extra swap belonging to some clause. 
	If we want to emphasize the fact that some swap belongs to
	some clause we say \emph{extra clause swap}.
	
	The remaining swaps can always be attributed to a variable-clause
	pair. As we fix the clause under consideration, we will
	further attribute every swap to either the \emph{satisfying side}
	 or the \emph{unsatisfying side}. Formally, this side
	is defined by the movement of the token labeled $C$. 
	(This is even true, if the player tries to cheat.)
	
%	Next we study the extra swaps taking place at the second row
%	in Figure~\ref{fig:TRG}. Variable $x$ does not satisfy $C$ and
%	variable $y$ satisfies $C$.
%	Therefore, we will have an extra swap between vertex 
%	$4$ and $5$. We call this \emph{extra clause-swap}. 
%	In case that $x$ satisfies $C$, the extra clause swap will
%	take place between vertex $3$ and $4$.
%	In any case, we will have in total 
%	exactly $m$ extra clause swaps.
%	
%	At last we will have either 

	Consider again Figure~\ref{fig:desPath} and note that the total 
	number of extra swaps for clause $C = \{x,\overline{y}\}$ equals 
	four. One extra 
	swap on the unsatisfying side and three on the satisfying side.
	
	Thus we have $4m$ extra clause swaps  and  $n$ extra 
	outside swaps in total.
	
	Now, let us turn our attention again to cheating. There are
	three possible ways of cheating. 
	\begin{enumerate}
		\item \label{case:over} 
		A clause is \emph{oversatisfied}. That is that there are two
		or more variables satisfying $C$. 
		To be more precise, we say a variable satisfies a clause, 
		if the real tokens arriving at the clause-gadget are 
		at the position corresponding to an satisfying assignment,
		see Figure~\ref{fig:cheating2}
		
		\item \label{case:change}
		The assignment of some variable $x$ is changed from false
		to true or from true to false.
		\item \label{case:under} A clause $C$ is \emph{undersatisfied}. 
		That is, each variable 
		is assigned a value that does not satisfy $C$. \label{case:under}
	\end{enumerate}
	
		Case~\ref{case:over} is the easiest, as it turns out that cheating
		in this way is not possible without using at least $6$ extra swaps
		in our example clause $C =  \{x,\overline{y}\}$.
		See Figure~\ref{fig:cheating2}. 
		In the example variable $x$ and variable $y$ are both 
		satisfying $C$. Token $C$ can only go to one of the sides 
		and the other side becomes unsatisfying. 
		Without loss of generality we chose $x$ as the unsatisfying
		 variable. 
		This is most problematic for token $d_{xC}$, as it
		has only two ways to reach the vertex $d_{xC}$ at the bottom.
		One of these ways is displayed in Figure~\ref{fig:cheating2}.
		It can be checked easily that (in both cases) the total number of
		extra swaps in this case will be $6$. 
		(three on the unsatisfying side and three 
		on the satisfying side.)
		 
		In Case~\ref{case:change}, we observe that any
		change of assignment involves at least one extra swap,
		either of vertices $8-9$, $8-10$, $12-14$ or $13-14$.
		See also Figure~\ref{fig:cheating1}. Potentially this
		extra swap could save an outside swap. So it might have
		globally no cost at all.
		A change of the assignment might also make it possible to 
		satisfy some later clause, which might be otherwise
		not possible. 
		(Note that a swap at $16-17$ or $19-20$ would be outside
		the clause.)
		
		To prevent this we modify $\varphi$ by making every clause
		appear $n+1$ times.
		Thus if $\varphi$ was not satisfiable than for every 
		copy of the original $\varphi$, we have to make at least one
		reassignment. This costs at least $n+1$ extra swaps. 
		In total we could save at most $n$ extra outside
		swaps by the reassignment. Thus also in this way cheating
		is at least one more expensive.
		
		Case~\ref{case:under} is most tricky and requires some 
		further modification. See Figure~\ref{fig:cheating3}.
		Assume that the assignment of $x$ and $y$ both do not
		satisfy $C$. Then the token $C$ has to go to one of the sides,
		assume as in Figure~\ref{fig:cheating3} this is the side of
		variable $x$. This can be done in various ways. One of them
		is depicted in Figure~\ref{fig:cheating3}. Counting the number 
		of extra swaps we have $3$ on this side. 
		But this is the same number
		as if $x$ would honestly satisfying $C$.
		In order to make this way of cheating more expensive,
		note that every sequence of swaps uses one extra swaps
		between different layers. In our example $3-11$.
		We subdivide every edge between the second and the first layer.
		The extra vertex gets a dummy-token, 
		which wants to stay where it is.
		This will make every swap between the second and third layer
		by two swaps more expensive. 
		These additional two swaps
		are counted as extra swaps if and only if 
		the non-dummy swap were counted as extra swap before 
		the subdivision.
		
		Thus the total number of extra swaps for all other 
		scenarios does not change due to this subdivision,
		but this scenario costs $5$ extra swaps now for 
		and is thus more expensive.
		
		It is easy to see that it is pointless
		for the new dummy-vertices to wander around other than
		making swaps between the second and third row more expensive.
		 
\end{proof}

		\newpage
		
\begin{figure}[htbp]%
		\centering
	\includegraphics{DesiredPaths}%
	\caption{
	 Setting $x$ and $y$ to false, the corresponding variable-,
	 clause- and dummy-paths are displayed. 
	 The sequence of swaps results
	 by swapping the real tokens along these paths in any order.
	 }%
	\label{fig:desPath}%

\vspace{1cm}

	\includegraphics{CheatingOversatisfied}%
	\caption{If the clause is satisfied by two 
	or more variables on of them needs to behave in a different manner,
	to bring every real vertex to its target vertex.
	The unsatisfying side has two more extra
	swaps 
	The extra swaps are $10-8$, and $8-9$.}%
\label{fig:cheating2}%
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]%
		\centering	\includegraphics{CheatingChangeAssignment}%
	\caption{Change the assignment by cheating.
	The extra swap is $8-10$ and $13-14$.}%
\label{fig:cheating1}%

\vspace{1cm}

	\includegraphics{CheatingUnsatisfied}%
	\caption{If the clause is not satisfied by two 
	or more variables on of them needs to behave in a different manner,
	to bring every real vertex to its target vertex.
	We will swap along the red path and thereafter the green path.
	The three black vertices, are labeled by their start vertex.
	On the ``satisfying'' side we do three extra swaps. Namely, $8-9$
	$11-3$ and $3-4$. The last two have to be done in this order.
	This is the same number as if $x$ were satisfying.
	But note that one of the extra swaps is between two different
	layers. }%
	\label{fig:cheating3}%
\end{figure}
	
	
	
	
	



